Barycentric alignment for instance-level comparison of neural representations

Comparing representations across neural networks is challenging because representations admit symmetries, such as arbitrary reordering of units or rotations of activation space, that obscure underlying equivalence between models. We introduce a barycentric alignment framework that quotients out these nuisance symmetries to construct a universal embedding space across many models. Unlike existing similarity measures, which summarize relationships over entire stimulus sets, this framework enables similarity to be defined at the level of individual stimuli, revealing inputs that elicit convergent versus divergent representations across models. Using this instance-level notion of similarity, we identify systematic input properties that predict representational convergence versus divergence across vision and language model families. We also construct universal embedding spaces for brain representations across individuals and cortical regions, enabling instance-level comparison of representational agreement across stages of the human visual hierarchy. Finally, we apply the same barycentric alignment framework to purely unimodal vision and language models and find that post-hoc alignment into a shared space yields image text similarity scores that closely track human cross-modal judgments and approach the performance of contrastively trained vision-language models. This strikingly suggests that independently learned representations already share sufficient geometric structure for human-aligned cross-modal comparison. Together, these results show that resolving representational similarity at the level of individual stimuli reveals phenomena that cannot be detected by set-level comparison metrics.

==> barycenter.tex <==
% \subsection{Universal Embedding Framework}

We propose a \emph{barycentric alignment} framework to map representations from many models into a single shared embedding space while explicitly quotienting out \emph{nuisance symmetries}. Each model’s representation of the same stimulus set is treated as a point cloud whose coordinates are only identifiable up to transformations induced by architectural and training choices (e.g., rotations). By aligning all models to a common \emph{barycenter} under an appropriate invariance class, we obtain a universal space in which representations become directly comparable across models and can be compared at the level of individual stimuli.

\subsection{Symmetries and the choice of alignment - }

We treat two representations as equivalent if they are related by a transformation from a specified group $\mathcal{G}$. Formally, let $X_i \in \mathbb{R}^{n \times d}$ denote the representation matrix from model $i$, where rows correspond to $n$ stimuli and columns to $d$ features. We consider $X_i \sim X_j$ if and only if there exists a transformation $T \in \mathcal{G}$ such that $X_i$ can be approximated well with $X_j T$.

The choice of $\mathcal{G}$ reflects assumptions about which transformations preserve meaningful representational content. Permutation invariance ($\mathcal{G} = \mathcal{P}(d)$, the group of permutation matrices) captures the intuition that neuron ordering is arbitrary. Orthogonal invariance ($\mathcal{G} = O(d)$, the orthogonal group) additionally accounts for rotations and reflections of the activation space. Throughout this work, we adopt orthogonal invariance as our default equivalence relation, as it provides a principled middle ground: it quotients out rotational degrees of freedom while preserving the metric structure of the representation space. Critically, the orthogonal group consists of linear isometries, i.e., transformations that preserve Euclidean distances. This ensures that aligning representations via orthogonal transformations does not distort the geometric relationships among stimuli within each model's space.

\subsection{Barycentric Alignment via Procrustes Iteration}

Given $N$ models, each producing representations for the same set of $n$ training stimuli, we seek a common embedding space and a set of alignment transformations $\{T_i\}_{i=1}^N$ such that the aligned representations $\{X_i T_i\}$ are mutually consistent. We formulate this as the problem of computing the \emph{Procrustes barycenter} of the $N$ representation matrices, i.e., the mean shape in the quotient space induced by orthogonal equivalence. 

To ensure consistent dimensionality across models, we set $d = \max(d_1, \ldots, d_N)$, where $d_i$ denotes the original dimensionality of model $i$. Representations from models with $d_i < d$ are zero-padded to match the maximum dimensionality. We initialize the template $M^{(0)}$ as the arithmetic mean of the representations and then iterate the following procedure:

\textbf{Alignment step:} For each model $i$, compute the orthogonal Procrustes transformation $ T_i = \arg\min_{R \in O(d)} \|X_i R - M^{(t)}\|_F$,
    which admits a closed-form solution via the singular value decomposition.
    
\textbf{Update step:} Set $X_i^{(t)} \leftarrow X_i T_i$ and recompute the template as $M^{(t+1)} = \frac{1}{N} \sum_{i=1}^N X_i^{(t)}$.

This alternating procedure converges to a local minimum of the sum of squared Procrustes distances, yielding aligned representations that reside in a shared coordinate system. We stop early when $\|M^{(t+1)}-M^{(t)}\|_F/\|M^{(t)}\|_F<\varepsilon$. The resulting template $M$ can be interpreted as the Fr\'{e}chet mean of the $N$ representations under the Procrustes metric, the resulting barycenter coordinates constitute what we refer to as the \emph{universal embedding space} and $\{T_i\}$ provide model-specific maps into that space.

Algorithm~\ref{alg:procrustes-barycenter-training} summarizes the training phase. The $n$ training stimuli used to learn the alignment transformations are held separate from the test stimuli used for inference.


\subsection{Inference and stimulus-wise agreement.}
Given a new set of $m$ test stimuli, each model produces representations $Y_i \in \mathbb{R}^{m \times d}, \qquad i=1,\dots,N$,
which we project into the universal space via the learned transforms: $Y_i' = Y_i T_i$.
For each test stimulus $j\in\{1,\dots,m\}$, we then quantify representational agreement by averaging pairwise similarity across the aligned representations: $S_j = \frac{1}{N(N-1)}\sum_{p\neq q} \mathrm{SIM}\!\left(Y'_{p j},\, Y'_{q j}\right)$,
where $Y'_{p j}$ denotes the row of $Y_p'$ corresponding to stimulus $j$. The similarity function is left generic; unless otherwise stated, we use cosine similarity throughout.
Throughout, we refer to this stimulus-wise representational agreement as the \emph{instance-level representational consistency score}, which quantifies the extent to which a stimulus admits a consistent representation across models after quotienting out nuisance symmetries.



